Explainable Abuse Detection as Intent Classification and Slot Filling

To proactively offer social media users a safe online experience, there is a need for systems that can detect harmful posts and promptly alert platform moderators. In order to guarantee the enforcement of a consistent policy, moderators are provided with detailed guidelines. In contrast, most state-of-the-art models learn what abuse is from labelled examples and as a result base their predictions on spurious cues, such as the presence of group identifiers, which can be unreliable. In this work we introduce the concept of policy-aware abuse detection, abandoning the unrealistic expectation that systems can reliably learn which phenomena constitute abuse from inspecting the data alone. We propose a machine-friendly representation of the policy that moderators wish to enforce, by breaking it down into a collection of intents and slots. We collect and annotate a dataset of 3,535 English posts with such slots, and show how architectures for intent classification and slot filling can be used for abuse detection, while providing a rationale for model decisions.

==> content/08_ethical_statement.tex <==
% How about annotators pay?
%Policy-specificity is not only a limitation, as it represents a defense from dual use. In fact, our approach cannot be used directly to enforce an unethical policy, as policy-specific modelling and annotations would be required.

To protect annotators from exposure to hateful content, we tagged our project with the ``offensive content'' label on Amazon Mechanical Turk, put a warning in the task title, and asked for consent twice (first at the end of the information sheet, and then with a one-sentence checkbox). Annotators were presented with small batches of 30 sentences, and invited to take a break at the end of each session. They were also offered the option to quit anytime during the session, or to abandon the study at any point. A reminder to seek for help in case they experienced distress was provided at the beginning of each session. The study was approved by the relevant ethics committee (details removed for anonymous peer review).

%Our data annotation process was run adding labels to an already public collection of posts. Our added annotations contain span-level tags (e.g., \texttt{Target}) together with demographic information of the annotator who produced the labels. For the annotators, we collect all and only the information necessary to identify whether the annotator is also a target of the annotated post. The purpose is to enable further research in online hate, as the development of algorithms for matching posts to the most suitable human moderator. Personal information are explicitly asked to the annotators, who can decide for each question whether to provide an answer or not. Data is then stored associated to an artificial annotator ID, and not the real one. A mapping between artificial and real IDs is kept in a separate table for payment purposes; at the time of writing, the table has been deleted.

==> content/old_03_policy_modelling.tex <==
% 4. First explain what our approach is (i.e., why we need to decompose the policy, we could already answer the question above keeping the whole policy text as input)
%     1. Write about explainability and everything
% 5. Policy choice and modelling:
%     1. AT policy: non-commercial, but similar to Hate Speech sections in Social Media policies
%     2. Decompose policy into atomic rules
%     3. Model rules as a conjunction of conditions
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|l|l}
\toprule
\textbf{Rule} & \textbf{Definition} & \textbf{Modelling} & \textbf{Example}\\
\midrule
Dehumanisation & \multirow{3}{*}{\shortstack[l]{Posts containing dehumanising comparisons\\ targeted to an individual or group based on their\\ protected characteristics violate the policy.}} & \multirow{3}{*}{\shortstack[l]{\textit{Target}$(s_1) \, \land$ \\ \textit{ProtectedCharacteristic}($s_2) \, \land$ \\ \textit{DehumanisingComparison}$(s_3)$}} & \multirow{3}{*}{\shortstack[l]{\textit{Target}$(\text{Immigrants}) \, \land$ \\ \textit{ProtectedCharacteristic}($\text{Immigrants}) \, \land$ \\ \textit{DehumanisingComparison}$(\text{are parasites})$}}\\
& & & \\
& & & \\
\midrule
%
Threatening & \multirow{3}{*}{\shortstack[l]{Posts containing threatening language\\ targeted to an individual or group based on their\\ protected characteristics violate the policy.}} & \multirow{3}{*}{\shortstack[l]{\textit{Target}$(s_1) \, \land$ \\ \textit{ProtectedCharacteristic}($s_2) \, \land$ \\ \textit{ThreateningSpeech}$(s_3)$}} & \multirow{3}{*}{\shortstack[l]{\textit{Target}$(\text{Women}) \, \land$ \\ \textit{ProtectedCharacteristic}($\text{Women}) \, \land$ \\ \textit{ThreateningSpeech}$(\text{should be killed})$}}\\
%
& & & \\
& & & \\
\midrule
Derogation & \multirow{3}{*}{\shortstack[l]{Posts containing derogatory terms or insults\\ targeted to an individual or group based on their\\ protected characteristics violate the policy.}} & \multirow{3}{*}{\shortstack[l]{\textit{Target}$(s_1) \, \land$ \\ \textit{ProtectedCharacteristic}($s_2) \, \land$ \\ \textit{DerogatoryOpinion}$(s_3)$}} & \multirow{3}{*}{\shortstack[l]{\textit{Target}$(\text{Polish people}) \, \land$ \\ \textit{ProtectedCharacteristic}($\text{Polish}) \, \land$ \\ \textit{DerogatoryOpinion}$(\text{are so nasty})$}}\\
& & & \\
& & & \\
\midrule
Animosity & \multirow{3}{*}{\shortstack[l]{Posts containing \textit{implicit} abusive language\\ targeted to an individual or group based on their\\ protected characteristics violate the policy.}} & \multirow{3}{*}{\shortstack[l]{\textit{Target}$(s_1) \, \land$ \\ \textit{ProtectedCharacteristic}($s_2) \, \land$ \\ \textit{NegativeOpinion}$(s_3)$}} & \multirow{3}{*}{\shortstack[l]{\textit{Target}$(\text{a breastfeeding woman}) \, \land$ \\ \textit{ProtectedCharacteristic}($\text{she}) \, \land$ \\ \textit{NegativeOpinion}$(\text{can do it at home})$}}\\
& & & \\
& & & \\
\midrule
Pro Hate Crime & \multirow{2}{*}{\shortstack[l]{Posts that glorify, support or deny hateful\\ actions, events, organisations and individuals.}} & \multirow{2}{*}{\shortstack[l]{\textit{HateEntity}$(s_1) \, \land$ \\ \textit{Support}($s_2)$}} & \multirow{2}{*}{\shortstack[l]{\textit{HateEntity}$(\text{Hitler}) \, \land$ \\ \textit{Support}($\text{was right all along})$}}\\
& & & \\
\bottomrule
\end{tabular}}
\caption{
Definition and modelling of each policy rule. Note that \texttt{ProtectedCharacteristic} models the phrase ``\textit{based} on their protected characteristics'', and therefore encodes a causality effect.
\label{tab:policy-modelling}}
\end{table*}%
%
The generation of explanations that are tailored to an input post $p$ requires detection systems to be able to reason over the policy content. To facilitate this process, we suggest to decompose the policy into a collection of atomic rules $R$, and represent each rule $r_i \in R$ as a conjunction of properties.
As a case-study, we choose to model the codebook\footnote{\url{https://github.com/bvidgen/Dynamically-Generated-Hate-Speech-Dataset}} for hate speech annotations designed by the Alan Turing Institute \cite{2021-vidgen-lftw}. Although we intentionally choose to work with a policy for non-commercial purposes, this policy is very similar to the guidelines that social media platforms provide to moderators and users\footnote{e.g., \url{https://transparency.fb.com/en-gb/policies/community-standards/hate-speech}}. We extract a rule from each section of the policy, and model each rule $r$ as a conjunction of properties:
% $$r_i \coloneqq P_1(s_1) \land \ldots \land P_{|r_i|}(s_{|r_i|})$$
% where $P_j$ is a relation over the set of subsequences of $p$ and $|r_i|$ is the number of properties in $r_i$ (see Table~\ref{tab:policy-modelling}).
\begin{equation}
    r \iff \forall P \in \delta(r) \enspace \exists \, s \in S(p): \, P(s)
\end{equation}
where $\delta(r)$ is the set of relations in the modelling of $r$, and $S(p)$ is the set of non-empty subsequences of $p$ (see Table~\ref{tab:policy-modelling}).
Note that commonsense knowledge is required to decide whether $P(s)$ holds true. For instance, \texttt{ThreateningSpeech(}\textit{dog}\texttt{)} is false, while \texttt{ThreateningSpeech(}\textit{should be killed}\texttt{)} is true. If $r$ holds (i.e. if a non-empty subsequence was found for each property such that all properties hold true), then the post $p$ violates the rule $r$. Besides being more machine-friendly and yet human readable, the described modelling has the further advantage of reducing the amount of task-specific data, and in particular of abusive instances, needed for training. In fact, decomposing rules into a conjunction of relations enables models to learn such relations even from non-abusive instances (e.g., by learning \texttt{Target} and \texttt{DehumanisingComparison} from \textit{``Artists are parasites''}). This is of crucial importance in this domain, since in absolute terms, abusive posts are (luckily) relatively infrequent compared with non-abusive posts \cite{2018-founta-abusive}, and most harmful contents is deleted by moderators upon detection.

\paragraph{Modelling counter speech} To enable models to correctly recognise posts that quote hate speech, but whose authors clearly distance themselves from the harmful message, we extend the modelling above with a new relation encoding the author's stance. For instance, the post \textit{``It's nonsense to say that Polish people are nasty''} contains a target of a derogatory opinion which is based on a protected characteristic of the target. All relations in the definition of the \texttt{Derogation} rule are satisfied, but the post should not be labelled as abusive as the author is reacting to the hateful message. To handle this form of counter speech (i.e., speech that directly counters hate, for example by presenting facts or reacting with humour \cite{2019-mathew-thou}) we define the relation \texttt{NegativeStance} over the set of subsequences of the input post $p$ and modify the classification rule as follows:
% $$r_i \iff r_i \land \neg \, NegativeStance(x)$$
\begin{align}
\begin{split}
    \label{eq:classification}
    r \iff & \forall P \in \delta(r) \enspace \exists \, s \in S(p): \, P(s) \enspace \land  \\ & \nexists \, s  \in S(p): \, NegativeStance(s)
\end{split}
\end{align}
This enables models to recognise \textit{``It's nonsense''} as the author's negative stance, and therefore to correctly classify the post as not hateful.
